Neural Embedding: Learning the Embedding of the Manifold of Physics Data

In this paper, we present a method of embedding physics data manifolds with metric structure into lower dimensional spaces with simpler metrics, such as Euclidean and Hyperbolic spaces. We then demonstrate that it can be a powerful step in the data analysis pipeline for many applications. Using progressively more realistic simulated collisions at the Large Hadron Collider, we show that this embedding approach learns the underlying latent structure. With the notion of volume in Euclidean spaces, we provide for the first time a viable solution to quantifying the true search capability of model agnostic search algorithms in collider physics (i.e. anomaly detection). Finally, we discuss how the ideas presented in this paper can be employed to solve many practical challenges that require the extraction of physically meaningful representations from information in complex high dimensional datasets.

==> acknowledgements.tex <==
P.H. acknowledges support by DOE grant de-sc0021943 and NSF CSSI award #1934700. SEP acknowledges support by DOE grant DE-SC0021225, and the Institute for Fundamental Interactions and Artificial Intelligence (NSF Award  #2019786). 

==> discussion.tex <==




==> jetexamples_temp.tex <==
Some of the examples of jets visualized by plotting each constituent in the $\eta-\phi$ plane with circles of sizes proportional to its $\pt$ is shown. 

\subsection{Simple Toy Jet}
\label{subsec:simpletoyjet_examples}



\begin{figure}[!htbp]
\centering
\includegraphics[width=.48\linewidth]{images/Examples_SimpleToyJet_1p.pdf}
\caption{ Samples of simple toy jet, 1-prong(QCD)
}
\label{fig:samplesimpletoyjet1p}
\end{figure}

\begin{figure}[!htbp]
\centering
\includegraphics[width=.48\linewidth]{images/Examples_SimpleToyJet_2p.pdf}
\caption{ Samples of simple toy jet, 2-prong
}
\label{fig:samplesimpletoyjet2p}
\end{figure}

\begin{figure}[!htbp]
\centering
\includegraphics[width=.48\linewidth]{images/Examples_SimpleToyJet_3p.pdf}
\caption{ Samples of simple toy jet, 3-prong
}
\label{fig:samplesimpletoyjet3p}
\end{figure}

\begin{figure}[!htbp]
\centering
\includegraphics[width=.48\linewidth]{images/Examples_SimpleToyJet_4p.pdf}
\caption{ Samples of simple toy jet, 4-prong
}
\label{fig:samplesimpletoyjet4p}
\end{figure}











\subsection{Realistic Toy Jet}
\label{subsec:realistictoyjet_examples}

\begin{figure}[!htbp]
\centering
\includegraphics[width=.48\linewidth]{images/Examples_RealisticToyJet_1p.pdf}
\caption{ Samples of realistic toy jet, 1-prong(QCD)
}
\label{fig:samplerealistictoyjet_1p}
\end{figure}

\begin{figure}[!htbp]
\centering
\includegraphics[width=.48\linewidth]{images/Examples_RealisticToyJet_2p.pdf}
\caption{ Samples of realistic toy jet, 2-prong
}
\label{fig:samplerealistictoyjet_2p}
\end{figure}

\begin{figure}[!htbp]
\centering
\includegraphics[width=.48\linewidth]{images/Examples-RealisticToyJet_3p.pdf}
\caption{ Samples of realistic toy jet, 3-prong
}
\label{fig:samplerealistictoyjet_3p}
\end{figure}


\begin{figure}[!htbp]
\centering
\includegraphics[width=.48\linewidth]{images/Examples_RealisticToyJet_4p.pdf}
\caption{ Samples of realistic toy jet, 4-prong
}
\label{fig:samplerealistictoyjet_4p}
\end{figure}




\subsection{Simulated Jet}
\label{subsec:simulatedjet_examples}



\begin{figure}[!htbp]
\centering
\includegraphics[width=.48\linewidth]{images/Examples_SimulatedJet_QCD.pdf}
\caption{ Samples of simulated jet, QCD
}
\label{fig:samplesimulatedjet_1p}
\end{figure}

\begin{figure}[!htbp]
\centering
\includegraphics[width=.48\linewidth]{images/Examples_SimulatedJet_2p.pdf}
\caption{ Samples of simulated jet, 2-prong 170 $\GeV$
}
\label{fig:samplesimulatedjet_2p}
\end{figure}

\begin{figure}[!htbp]
\centering
\includegraphics[width=.48\linewidth]{images/Examples_SimulatedJet_3p.pdf}
\caption{ Samples of simulated jet, 3-prong 170 $\GeV$
}
\label{fig:samplesimulatedjet_3p}
\end{figure}


\begin{figure}[!htbp]
\centering
\includegraphics[width=.48\linewidth]{images/Examples_SimulatedJet_4p.pdf}
\caption{ Samples of simulated jet, 4-prong 170 $\GeV$
}
\label{fig:samplesimulatedjet_4p}
\end{figure}



==> temp_problem_setting.tex <==
Suppose we have a metric space $(\mathcal{X}, d)$ of collider events, where $\mathcal{X}$ is a space of collider events and $d$ is a metric defined as , and we want to learn a mapping that satisfies a low distortion. 



And consider a map $\phi: (\mathcal{X},d_{\mathcal{X}}) \rightarrow (\mathcal{Y}, d_\mathcal{Y}$) that satisfies a low distortion, namely it satisfies the relation
\begin{equation}
\begin{aligned}
\forall u,v \in \mathcal{X}, \: L\cdot d_{\mathcal{Y}}(\phi(u),\phi(v)) < d_\mathcal{X}(u,v) < C\cdot d_\mathcal{Y}(\phi(u),\phi(v)) 
\end{aligned}
\end{equation}
For some $L>0$ and $C \geq 0$. The distortion is the smallest $C$ such that the above relation holds. 


If we consider an embedding into a euclidean space with a $l_2$-norm, 
\begin{equation}
\begin{aligned}
\phi: (\mathcal{X}, W_p() ) \rightarrow (\mathbb{R}^2, l_2)
\end{aligned}
\end{equation}


Treating data points as discrete measure on the Wasserstein space, we can also consider the Wasserstein embedding ~\cite{frogner2019learning}, \begin{equation}
\begin{aligned}
\phi: (\mathcal{X}, W_p() ) \rightarrow ()
\end{aligned}
\end{equation}


Many metrics have been proposed on the collider events, many based on Optimal Transport. such as Energy mover's distance based on Wasserstein distance, and Hellinger distance
If we consider the metric to be a Wasserstein metric, like in the EMD paper, square hellinger distance


\subsection{Network architecture}

We will learn to approximate the embedding function by deep neural network with strong expressive power. For the mnist case, we used CNN and for toy jet generator represented as constituent particles, we used transformer architecture. 


network architecture
We will learn the embedding function by gradient descent on a pair objective function. Transformers 

The mapping is represented as a equation 


The training objective is to learn the embedding function between the data space equipped with a certain metric, 
to a low dimensional euclidean space equipped with a euclidean distance. 

For instance, 
If we are dealing with jets represented as $N$ number of its highest transverse momentum components each with $(\pt, \eta, \phi)$ information, then we can equip this space of jets which is a subset of $\mathbb{R}^{3N}$ to the euclidean space $\mathbb{R}^{2}$ with $l_2$-norm. 


in the form of where the distance is 






In our specific case, we let the embedding to be between 


We will learn the embedding function through gradient descent 

Is a common research topic, frechet embedding 

$\phi(x)$


The training objective can be formulated in multiple ways. 
Training objective is pair triplet n pair

The embedding function itself has to be expressive to embed different structures of data with minimum distortion. 




The embedding can change according to the data we need to process. 
We chose embedding function to be transformer with self encoding, and in MNIST setting we choose it to be a CNN. 

solomon embedding 


TSNE, etc does not preserve the distance


Test on prongs that seen in training :
Test on mass points that not seen in training:



We tested the embedding procedure into the low dimensional manifold in three different settings. 

First is the MNIST for illustrative purposes. 

Second is the toy jet generator described in detail in a previous section. 



We can also view it from another perspective, which is building space from distance between pairs of points. The net effect of embedding is that we can build space from raw optimal transport distances between inputs
where we can do a lot of things and the space which is  very useful 


There are many different distance on space of collider events. (EMD,,, etc ) 

Euclidean embedding discrete measure


Systematically measured distortion as in ~\cite{VakandaraDistortion}
